Adaptive Sparsity Level during Training for Efficient Time Series Forecasting with Transformers

Efficient time series forecasting has become critical for real-world applications, particularly with deep neural networks (DNNs). Efficiency in DNNs can be achieved through sparse connectivity and reducing the model size. However, finding the sparsity level automatically during training remains challenging due to the heterogeneity in the loss-sparsity tradeoffs across the datasets. In this paper, we propose \enquote{\textbf{P}runing with \textbf{A}daptive \textbf{S}parsity \textbf{L}evel} (\textbf{PALS}), to automatically seek a decent balance between loss and sparsity, all without the need for a predefined sparsity level. PALS draws inspiration from sparse training and during-training methods. It introduces the novel "expand" mechanism in training sparse neural networks, allowing the model to dynamically shrink, expand, or remain stable to find a proper sparsity level. In this paper, we focus on achieving efficiency in transformers known for their excellent time series forecasting performance but high computational cost. Nevertheless, PALS can be applied directly to any DNN. To this aim, we demonstrate its effectiveness also on the DLinear model. Experimental results on six benchmark datasets and five state-of-the-art (SOTA) transformer variants show that PALS substantially reduces model size while maintaining comparable performance to the dense model. More interestingly, PALS even outperforms the dense model, in \textcolor{blue}{12} and \textcolor{blue}{14} cases out of 30 cases in terms of MSE and MAE loss, respectively, while reducing \textcolor{blue}{65\%} parameter count and \textcolor{blue}{63\%} FLOPs on average. Our code and supplementary material are available on Github\footnote{\tiny \url{https://github.com/zahraatashgahi/PALS}}.

==> assets/tables/adapt_tuned_detailed_all.tex <==

\begin{table*}[!t]




\caption{Comparison on the benchmark Datasets for prediction length $H \in \{96, 192, 336, 720\}$ (except for the Illness dataset for which $H \in \{24, 36, 48, 60\}$). For each model, the performance of the original (Dense) and the pruned model using PALS is presented in terms of MSE and parameter count. The difference between the results compared to the dense counterpart is shown in parenthesis as \% (\textcolor{blue}{blue} indicates improvement in the results compared to the dense model). \textbf{Bold} entries are the best performer in each experiment among various models. }\label{tab:results_all}
\centering
\resizebox{1.1\textwidth}{!}{% <------ Don't forget this %
\begin{tabular}{@{\hskip 0.0in}c@{\hskip 0.03in}c@{\hskip 0.03in}|@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}|@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}|@{\hskip 0.03in}c@{\hskip 0.03in}@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c|c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}|@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c}
\toprule
\bt \multirow{3}{*}{\rotatebox[origin=c]{90}{Datasets}}& \bt \multirow{3}{*}{$H$} &\multicolumn{4}{c}{NSTransformer}| &\multicolumn{4}{c}{FEDformer}| &\multicolumn{4}{c}{Autoformer}|&\multicolumn{4}{c}{Informer}| &\multicolumn{4}{c}{Transformer}\\

&&\multicolumn{2}{c}{Dense} &\multicolumn{2}{c}{+PALS}       &\multicolumn{2}{c}{Dense} &\multicolumn{2}{c}{+PALS}  &\multicolumn{2}{c}{Dense} &\multicolumn{2}{c}{+PALS}       &\multicolumn{2}{c}{Dense} &\multicolumn{2}{c}{+PALS} &\multicolumn{2}{c}{Dense} &\multicolumn{2}{c}{+PALS}\\ 


& &MSE &\#Param  &MSE &\#Param       &MSE &\#Param  &MSE &\#Param       &MSE &\#Param  &MSE &\#Param          &MSE &\#Param  &MSE &\#Param      &MSE &\#Param  &MSE &\#Param  \\
\midrule 

\multirow{4}{*}{\rotatebox[origin=c]{90}{Electricity}}& 96& \pmb{0.170}& 12.2& 0.195 (\textcolor{black}{14.3\%} $\uparrow$)& 2.6  (\textcolor{black}{78.2\%} $\downarrow$)& 0.187& 19.5& 0.203 (\textcolor{black}{8.6\%} $\uparrow$)& 4.4  (\textcolor{black}{77.3\%} $\downarrow$)& 0.207& 12.1& 0.206 (\textcolor{blue}{0.4\%} $\downarrow$)& 5.3  (\textcolor{black}{56.2\%} $\downarrow$)& 0.333& 12.5& 0.347 (\textcolor{black}{4.3\%} $\uparrow$)& 1.2  (\textcolor{black}{90.1\%} $\downarrow$)& 0.257& 11.7& 0.282 (\textcolor{black}{9.6\%} $\uparrow$)& 3.0  (\textcolor{black}{73.9\%} $\downarrow$) \\
& 192& \pmb{0.186}& 12.2& 0.204 (\textcolor{black}{10.0\%} $\uparrow$)& 1.9  (\textcolor{black}{84.3\%} $\downarrow$)& 0.196& 19.5& 0.212 (\textcolor{black}{8.3\%} $\uparrow$)& 2.8  (\textcolor{black}{85.9\%} $\downarrow$)& 0.219& 12.1& 0.241 (\textcolor{black}{9.9\%} $\uparrow$)& 2.8  (\textcolor{black}{76.7\%} $\downarrow$)& 0.347& 12.5& 0.373 (\textcolor{black}{7.4\%} $\uparrow$)& 2.0  (\textcolor{black}{84.2\%} $\downarrow$)& 0.270& 11.7& 0.300 (\textcolor{black}{11.3\%} $\uparrow$)& 1.4  (\textcolor{black}{87.8\%} $\downarrow$) \\
& 336& \pmb{0.198}& 11.9& 0.220 (\textcolor{black}{11.1\%} $\uparrow$)& 1.2  (\textcolor{black}{90.0\%} $\downarrow$)& 0.209& 19.5& 0.225 (\textcolor{black}{7.7\%} $\uparrow$)& 1.9  (\textcolor{black}{90.1\%} $\downarrow$)& 0.239& 12.1& 0.270 (\textcolor{black}{13.2\%} $\uparrow$)& 1.2  (\textcolor{black}{90.2\%} $\downarrow$)& 0.352& 12.5& 0.405 (\textcolor{black}{15.2\%} $\uparrow$)& 1.2  (\textcolor{black}{90.1\%} $\downarrow$)& 0.291& 11.7& 0.315 (\textcolor{black}{8.2\%} $\uparrow$)& 1.3  (\textcolor{black}{88.5\%} $\downarrow$) \\
& 720& \pmb{0.222}& 11.9& 0.241 (\textcolor{black}{8.6\%} $\uparrow$)& 3.2  (\textcolor{black}{73.5\%} $\downarrow$)& 0.238& 19.5& 0.265 (\textcolor{black}{11.0\%} $\uparrow$)& 2.8  (\textcolor{black}{85.4\%} $\downarrow$)& 0.279& 12.1& 0.315 (\textcolor{black}{12.7\%} $\uparrow$)& 1.5  (\textcolor{black}{87.7\%} $\downarrow$)& 0.393& 12.5& 0.569 (\textcolor{black}{44.8\%} $\uparrow$)& 1.2  (\textcolor{black}{90.0\%} $\downarrow$)& 0.307& 11.7& 0.346 (\textcolor{black}{12.7\%} $\uparrow$)& 4.3  (\textcolor{black}{62.9\%} $\downarrow$) \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm2}}& 96& 0.241& 10.6& 0.244 (\textcolor{black}{1.0\%} $\uparrow$)& 4.1  (\textcolor{black}{61.0\%} $\downarrow$)& \pmb{0.190}& 17.9& 0.201 (\textcolor{black}{5.7\%} $\uparrow$)& 1.8  (\textcolor{black}{90.2\%} $\downarrow$)& 0.233& 10.5& 0.214 (\textcolor{blue}{7.9\%} $\downarrow$)& 1.0  (\textcolor{black}{90.1\%} $\downarrow$)& 0.485& 11.3& 0.371 (\textcolor{blue}{23.3\%} $\downarrow$)& 8.7  (\textcolor{black}{22.9\%} $\downarrow$)& 0.418& 10.5& 0.268 (\textcolor{blue}{35.8\%} $\downarrow$)& 1.0  (\textcolor{black}{90.8\%} $\downarrow$) \\
& 192& 0.387& 10.7& 0.480 (\textcolor{black}{24.1\%} $\uparrow$)& 3.7  (\textcolor{black}{65.6\%} $\downarrow$)& \pmb{0.259}& 17.9& 0.263 (\textcolor{black}{1.7\%} $\uparrow$)& 1.8  (\textcolor{black}{90.2\%} $\downarrow$)& 0.302& 10.5& 0.269 (\textcolor{blue}{10.8\%} $\downarrow$)& 1.0  (\textcolor{black}{90.4\%} $\downarrow$)& 0.742& 11.3& 0.777 (\textcolor{black}{4.7\%} $\uparrow$)& 4.1  (\textcolor{black}{63.6\%} $\downarrow$)& 1.093& 10.5& 0.527 (\textcolor{blue}{51.8\%} $\downarrow$)& 1.0  (\textcolor{black}{90.3\%} $\downarrow$) \\
& 336& 0.615& 10.6& 0.339 (\textcolor{blue}{44.9\%} $\downarrow$)& 1.0  (\textcolor{black}{90.2\%} $\downarrow$)& \pmb{0.320}& 17.9& 0.325 (\textcolor{black}{1.4\%} $\uparrow$)& 1.8  (\textcolor{black}{90.2\%} $\downarrow$)& 0.338& 10.5& 0.326 (\textcolor{blue}{3.4\%} $\downarrow$)& 1.0  (\textcolor{black}{90.2\%} $\downarrow$)& 1.400& 11.3& 1.084 (\textcolor{blue}{22.5\%} $\downarrow$)& 1.2  (\textcolor{black}{89.8\%} $\downarrow$)& 1.387& 10.5& 0.982 (\textcolor{blue}{29.2\%} $\downarrow$)& 2.6  (\textcolor{black}{75.2\%} $\downarrow$) \\
& 720& 0.734& 10.6& 0.439 (\textcolor{blue}{40.1\%} $\downarrow$)& 1.0  (\textcolor{black}{90.2\%} $\downarrow$)& 0.425& 17.9& 0.423 (\textcolor{blue}{0.4\%} $\downarrow$)& 1.8  (\textcolor{black}{90.1\%} $\downarrow$)& 0.463& 10.5& \pmb{0.417} (\textcolor{blue}{9.9\%} $\downarrow$)& 1.0  (\textcolor{black}{90.4\%} $\downarrow$)& 3.479& 11.3& 3.320 (\textcolor{blue}{4.5\%} $\downarrow$)& 7.1  (\textcolor{black}{37.4\%} $\downarrow$)& 3.018& 10.5& 2.561 (\textcolor{blue}{15.1\%} $\downarrow$)& 8.1  (\textcolor{black}{23.4\%} $\downarrow$) \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Exchange}}& 96& 0.124& 10.5& \pmb{0.116} (\textcolor{blue}{6.8\%} $\downarrow$)& 1.0  (\textcolor{black}{90.4\%} $\downarrow$)& 0.146& 17.9& 0.155 (\textcolor{black}{5.7\%} $\uparrow$)& 6.7  (\textcolor{black}{62.7\%} $\downarrow$)& 0.147& 10.5& 0.148 (\textcolor{black}{0.4\%} $\uparrow$)& 5.9  (\textcolor{black}{44.2\%} $\downarrow$)& 0.941& 11.3& 0.945 (\textcolor{black}{0.5\%} $\uparrow$)& 7.7  (\textcolor{black}{32.1\%} $\downarrow$)& 0.679& 10.5& 0.651 (\textcolor{blue}{4.2\%} $\downarrow$)& 7.2  (\textcolor{black}{31.6\%} $\downarrow$) \\
& 192& 0.243& 10.5& \pmb{0.233} (\textcolor{blue}{4.4\%} $\downarrow$)& 4.2  (\textcolor{black}{60.2\%} $\downarrow$)& 0.271& 17.9& 0.276 (\textcolor{black}{1.6\%} $\uparrow$)& 10.6  (\textcolor{black}{40.5\%} $\downarrow$)& 0.285& 10.5& 0.412 (\textcolor{black}{44.3\%} $\uparrow$)& 6.2  (\textcolor{black}{41.6\%} $\downarrow$)& 1.077& 11.3& 1.087 (\textcolor{black}{1.0\%} $\uparrow$)& 7.7  (\textcolor{black}{32.5\%} $\downarrow$)& 1.255& 10.5& 1.229 (\textcolor{blue}{2.0\%} $\downarrow$)& 7.0  (\textcolor{black}{33.5\%} $\downarrow$) \\
& 336& 0.462& 10.6& 0.459 (\textcolor{blue}{0.5\%} $\downarrow$)& 8.2  (\textcolor{black}{22.0\%} $\downarrow$)& \pmb{0.443}& 17.9& 0.447 (\textcolor{black}{0.9\%} $\uparrow$)& 11.9  (\textcolor{black}{33.2\%} $\downarrow$)& 0.772& 10.5& 0.695 (\textcolor{blue}{9.9\%} $\downarrow$)& 8.2  (\textcolor{black}{22.1\%} $\downarrow$)& 1.609& 11.3& 1.596 (\textcolor{blue}{0.8\%} $\downarrow$)& 9.2  (\textcolor{black}{19.1\%} $\downarrow$)& 1.565& 10.5& 1.588 (\textcolor{black}{1.5\%} $\uparrow$)& 6.3  (\textcolor{black}{40.5\%} $\downarrow$) \\
& 720& 1.336& 10.6& 1.156 (\textcolor{blue}{13.5\%} $\downarrow$)& 8.3  (\textcolor{black}{21.3\%} $\downarrow$)& 1.143& 17.9& 1.169 (\textcolor{black}{2.3\%} $\uparrow$)& 12.8  (\textcolor{black}{28.6\%} $\downarrow$)& \pmb{1.128}& 10.5& 1.206 (\textcolor{black}{6.9\%} $\uparrow$)& 8.1  (\textcolor{black}{23.0\%} $\downarrow$)& 2.747& 11.3& 2.497 (\textcolor{blue}{9.1\%} $\downarrow$)& 9.8  (\textcolor{black}{13.1\%} $\downarrow$)& 2.938& 10.5& 2.164 (\textcolor{blue}{26.3\%} $\downarrow$)& 5.9  (\textcolor{black}{44.4\%} $\downarrow$) \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Illness}}& 24& \pmb{2.555}& 10.5& 2.641 (\textcolor{black}{3.3\%} $\uparrow$)& 6.9  (\textcolor{black}{35.0\%} $\downarrow$)& 3.285& 13.1& 3.590 (\textcolor{black}{9.3\%} $\uparrow$)& 7.6  (\textcolor{black}{42.1\%} $\downarrow$)& 3.686& 10.5& 3.648 (\textcolor{blue}{1.0\%} $\downarrow$)& 7.5  (\textcolor{black}{29.2\%} $\downarrow$)& 5.361& 11.3& 5.412 (\textcolor{black}{1.0\%} $\uparrow$)& 7.9  (\textcolor{black}{29.9\%} $\downarrow$)& 4.740& 10.5& 4.739 (\textcolor{blue}{0.0\%} $\downarrow$)& 6.9  (\textcolor{black}{34.3\%} $\downarrow$) \\
& 36& \pmb{1.913}& 10.5& 2.111 (\textcolor{black}{10.4\%} $\uparrow$)& 7.9  (\textcolor{black}{25.4\%} $\downarrow$)& 2.682& 13.5& 2.835 (\textcolor{black}{5.7\%} $\uparrow$)& 8.5  (\textcolor{black}{36.7\%} $\downarrow$)& 2.799& 10.5& 3.118 (\textcolor{black}{11.4\%} $\uparrow$)& 6.9  (\textcolor{black}{34.8\%} $\downarrow$)& 5.304& 11.3& 5.239 (\textcolor{blue}{1.2\%} $\downarrow$)& 6.6  (\textcolor{black}{41.7\%} $\downarrow$)& 4.776& 10.5& 4.911 (\textcolor{black}{2.8\%} $\uparrow$)& 8.1  (\textcolor{black}{23.2\%} $\downarrow$) \\
& 48& \pmb{1.873}& 10.5& 2.186 (\textcolor{black}{16.7\%} $\uparrow$)& 7.8  (\textcolor{black}{25.6\%} $\downarrow$)& 2.585& 13.9& 2.762 (\textcolor{black}{6.9\%} $\uparrow$)& 8.8  (\textcolor{black}{36.4\%} $\downarrow$)& 2.990& 10.5& 3.017 (\textcolor{black}{0.9\%} $\uparrow$)& 5.3  (\textcolor{black}{49.3\%} $\downarrow$)& 5.187& 11.3& 5.064 (\textcolor{blue}{2.4\%} $\downarrow$)& 7.5  (\textcolor{black}{34.0\%} $\downarrow$)& 5.090& 10.5& 4.914 (\textcolor{blue}{3.5\%} $\downarrow$)& 7.7  (\textcolor{black}{26.5\%} $\downarrow$) \\
& 60& \pmb{2.209}& 10.5& 2.391 (\textcolor{black}{8.2\%} $\uparrow$)& 7.0  (\textcolor{black}{34.0\%} $\downarrow$)& 2.807& 14.3& 2.994 (\textcolor{black}{6.7\%} $\uparrow$)& 8.2  (\textcolor{black}{42.7\%} $\downarrow$)& 2.860& 10.5& 2.984 (\textcolor{black}{4.3\%} $\uparrow$)& 7.0  (\textcolor{black}{33.2\%} $\downarrow$)& 5.234& 11.3& 5.197 (\textcolor{blue}{0.7\%} $\downarrow$)& 7.5  (\textcolor{black}{34.1\%} $\downarrow$)& 5.162& 10.5& 5.070 (\textcolor{blue}{1.8\%} $\downarrow$)& 7.9  (\textcolor{black}{25.0\%} $\downarrow$) \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Traffic}}& 96& 0.608& 14.1& 0.641 (\textcolor{black}{5.4\%} $\uparrow$)& 4.3  (\textcolor{black}{69.6\%} $\downarrow$)& \pmb{0.581}& 22.3& 0.585 (\textcolor{black}{0.8\%} $\uparrow$)& 5.4  (\textcolor{black}{75.6\%} $\downarrow$)& 0.649& 14.9& 0.629 (\textcolor{blue}{3.1\%} $\downarrow$)& 5.2  (\textcolor{black}{65.2\%} $\downarrow$)& 0.724& 14.4& 0.744 (\textcolor{black}{2.7\%} $\uparrow$)& 1.5  (\textcolor{black}{89.3\%} $\downarrow$)& 0.646& 13.6& 0.677 (\textcolor{black}{4.8\%} $\uparrow$)& 3.7  (\textcolor{black}{72.8\%} $\downarrow$) \\
& 192& 0.623& 14.1& 0.660 (\textcolor{black}{5.9\%} $\uparrow$)& 4.3  (\textcolor{black}{69.4\%} $\downarrow$)& \pmb{0.605}& 22.3& 0.608 (\textcolor{black}{0.5\%} $\uparrow$)& 3.9  (\textcolor{black}{82.4\%} $\downarrow$)& 0.630& 14.9& 0.653 (\textcolor{black}{3.6\%} $\uparrow$)& 5.6  (\textcolor{black}{62.4\%} $\downarrow$)& 0.746& 14.4& 0.771 (\textcolor{black}{3.3\%} $\uparrow$)& 1.6  (\textcolor{black}{88.9\%} $\downarrow$)& 0.660& 13.6& 0.685 (\textcolor{black}{3.9\%} $\uparrow$)& 4.5  (\textcolor{black}{66.7\%} $\downarrow$) \\
& 336& 0.640& 14.6& 0.672 (\textcolor{black}{5.0\%} $\uparrow$)& 3.1  (\textcolor{black}{78.7\%} $\downarrow$)& 0.618& 22.3& 0.625 (\textcolor{black}{1.1\%} $\uparrow$)& 5.6  (\textcolor{black}{75.0\%} $\downarrow$)& \pmb{0.614}& 14.9& 0.649 (\textcolor{black}{5.7\%} $\uparrow$)& 3.5  (\textcolor{black}{76.8\%} $\downarrow$)& 0.830& 14.4& 0.907 (\textcolor{black}{9.3\%} $\uparrow$)& 1.7  (\textcolor{black}{88.1\%} $\downarrow$)& 0.668& 13.6& 0.687 (\textcolor{black}{2.8\%} $\uparrow$)& 3.2  (\textcolor{black}{76.5\%} $\downarrow$) \\
& 720& 0.658& 14.1& 0.687 (\textcolor{black}{4.5\%} $\uparrow$)& 5.3  (\textcolor{black}{62.4\%} $\downarrow$)& \pmb{0.634}& 22.3& 0.643 (\textcolor{black}{1.5\%} $\uparrow$)& 7.7  (\textcolor{black}{65.5\%} $\downarrow$)& 0.663& 14.9& 0.673 (\textcolor{black}{1.5\%} $\uparrow$)& 3.9  (\textcolor{black}{73.7\%} $\downarrow$)& 0.943& 14.4& 1.324 (\textcolor{black}{40.3\%} $\uparrow$)& 4.4  (\textcolor{black}{69.2\%} $\downarrow$)& 0.693& 13.6& 0.705 (\textcolor{black}{1.7\%} $\uparrow$)& 4.0  (\textcolor{black}{70.9\%} $\downarrow$) \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Weather}}& 96& 0.182& 10.8& \pmb{0.167} (\textcolor{blue}{8.0\%} $\downarrow$)& 1.0  (\textcolor{black}{90.3\%} $\downarrow$)& 0.240& 17.9& 0.214 (\textcolor{blue}{11.0\%} $\downarrow$)& 1.8  (\textcolor{black}{90.0\%} $\downarrow$)& 0.266& 10.6& 0.258 (\textcolor{blue}{2.9\%} $\downarrow$)& 1.1  (\textcolor{black}{90.0\%} $\downarrow$)& 0.375& 11.4& 0.349 (\textcolor{blue}{7.0\%} $\downarrow$)& 1.1  (\textcolor{black}{90.2\%} $\downarrow$)& 0.380& 10.6& 0.198 (\textcolor{blue}{47.8\%} $\downarrow$)& 1.0  (\textcolor{black}{90.1\%} $\downarrow$) \\
& 192& 0.247& 10.6& \pmb{0.220} (\textcolor{blue}{11.0\%} $\downarrow$)& 1.0  (\textcolor{black}{90.5\%} $\downarrow$)& 0.281& 17.9& 0.281 (\textcolor{blue}{0.0\%} $\downarrow$)& 1.8  (\textcolor{black}{90.0\%} $\downarrow$)& 0.304& 10.6& 0.306 (\textcolor{black}{0.7\%} $\uparrow$)& 1.0  (\textcolor{black}{90.4\%} $\downarrow$)& 0.512& 11.4& 0.469 (\textcolor{blue}{8.4\%} $\downarrow$)& 2.6  (\textcolor{black}{76.8\%} $\downarrow$)& 0.584& 10.6& 0.282 (\textcolor{blue}{51.6\%} $\downarrow$)& 1.0  (\textcolor{black}{90.1\%} $\downarrow$) \\
& 336& 0.329& 10.6& \pmb{0.293} (\textcolor{blue}{10.9\%} $\downarrow$)& 1.0  (\textcolor{black}{90.1\%} $\downarrow$)& 0.367& 17.9& 0.337 (\textcolor{blue}{8.0\%} $\downarrow$)& 1.8  (\textcolor{black}{90.0\%} $\downarrow$)& 0.360& 10.6& 0.375 (\textcolor{black}{4.1\%} $\uparrow$)& 1.0  (\textcolor{black}{90.1\%} $\downarrow$)& 0.604& 11.4& 0.560 (\textcolor{blue}{7.3\%} $\downarrow$)& 4.2  (\textcolor{black}{63.0\%} $\downarrow$)& 0.684& 10.6& 0.343 (\textcolor{blue}{49.9\%} $\downarrow$)& 1.0  (\textcolor{black}{90.1\%} $\downarrow$) \\
& 720& 0.410& 10.6& \pmb{0.368} (\textcolor{blue}{10.1\%} $\downarrow$)& 1.0  (\textcolor{black}{90.2\%} $\downarrow$)& 0.395& 17.9& 0.410 (\textcolor{black}{3.9\%} $\uparrow$)& 1.8  (\textcolor{black}{90.1\%} $\downarrow$)& 0.423& 10.6& 0.416 (\textcolor{blue}{1.7\%} $\downarrow$)& 2.1  (\textcolor{black}{80.3\%} $\downarrow$)& 0.987& 11.4& 1.400 (\textcolor{black}{41.8\%} $\uparrow$)& 9.4  (\textcolor{black}{17.6\%} $\downarrow$)& 0.930& 10.6& 0.476 (\textcolor{blue}{48.9\%} $\downarrow$)& 1.0  (\textcolor{black}{90.4\%} $\downarrow$) \\


\bottomrule
\end{tabular}}


\end{table*}





==> assets/tables/summary_comparison_models_all.tex <==


\begin{table*}[!h]
\begin{scriptsize}

\caption{Comparison on the benchmark Datasets.}\label{tab:summary_results_all}
\begin{center}
\scalebox{0.8}{
\begin{tabular}{c| c@{\hskip 0.04in}c@{\hskip 0.04in}c|c@{\hskip 0.04in}c@{\hskip 0.04in}c|c@{\hskip 0.04in}c@{\hskip 0.04in}c|c@{\hskip 0.04in}c@{\hskip 0.04in}c|c@{\hskip 0.04in}c@{\hskip 0.04in}c|c@{\hskip 0.04in}c@{\hskip 0.04in}c@{\hskip 0.04in}c}
%\begin{tabular}{@{\hskip 0.08in}c@{\hskip 0.08in}c@{\hskip 0.08in}c@{\hskip 0.08in}c@{\hskip 0.08in}c@{\hskip 0.08in}c@{\hskip 0.08in}c@{\hskip 0.08in}c@{\hskip 0.08in}c@{\hskip 0.08in}c@{\hskip 0.08in}c@{\hskip 0.08in}c@{\hskip 0.08in}c}
\toprule
\bt Model  &\multicolumn{3}{c}{Electricity} & \multicolumn{3}{c}{ETTm2}  & \multicolumn{3}{c}{Exchange} & \multicolumn{3}{c}{Illness}  & \multicolumn{3}{c}{Traffic}  & \multicolumn{3}{c}{Weather}\\


& MSE &MAE &\#Params & MSE &MAE &\#Params & MSE &MAE &\#Params & MSE &MAE  &\#Params  & MSE &MAE &\#Params  & MSE &MAE  &\#Params \\
\midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{19}{c}{Sparse Model Hidden Size = 256, Init Density = 1}\\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


NSTransformer& \textbf{0.194}& \textbf{0.296}& 11.9& \textbf{0.505}& \textbf{0.438}& 10.7& 0.541& 0.487& 10.6& \textbf{2.138}& \textbf{0.919}& 10.5& \textbf{0.632}& \textbf{0.344}& 14.1& \textbf{0.292}& \textbf{0.313}& 10.6 \\
+PALS& 0.248& 0.342& \textbf{1.3}& 10.000& 10.000& \textbf{10.0}& \textbf{0.500}& \textbf{0.473}& \textbf{4.2}& 2.687& 1.049& \textbf{2.7}& 0.687& 0.389& \textbf{2.6}& 10.000& 10.000& \textbf{10.0} \\
Difference& 27.6\% $\uparrow$& 15.6\% $\uparrow$& \textcolor{blue}{\textbf{88.9\% $\downarrow$}}& 1881.4\% $\uparrow$& 2185.6\% $\uparrow$& \textcolor{blue}{\textbf{6.6\% $\downarrow$}}& \textcolor{blue}{\textbf{7.7\% $\downarrow$}}& \textcolor{blue}{\textbf{2.8\% $\downarrow$}}& \textcolor{blue}{\textbf{60.0\% $\downarrow$}}& 25.7\% $\uparrow$& 14.2\% $\uparrow$& \textcolor{blue}{\textbf{74.4\% $\downarrow$}}& 8.6\% $\uparrow$& 13.1\% $\uparrow$& \textcolor{blue}{\textbf{81.4\% $\downarrow$}}& 3328.0\% $\uparrow$& 3090.3\% $\uparrow$& \textcolor{blue}{\textbf{6.1\% $\downarrow$}} \\
\midrule

FEDformer& \textbf{0.207}& \textbf{0.321}& 19.5& \textbf{0.298}& \textbf{0.347}& 17.9& \textbf{0.501}& 0.493& 17.9& \textbf{2.840}& \textbf{1.137}& 14.3& \textbf{0.609}& \textbf{0.377}& 22.3& \textbf{0.320}& \textbf{0.367}& 17.9 \\
+PALS& 0.250& 0.357& \textbf{1.7}& 10.000& 10.000& \textbf{10.0}& 0.504& \textbf{0.492}& \textbf{2.9}& 3.589& 1.327& \textbf{3.0}& 0.636& 0.397& \textbf{3.3}& 10.000& 10.000& \textbf{10.0} \\
Difference& 20.3\% $\uparrow$& 11.2\% $\uparrow$& \textcolor{blue}{\textbf{91.3\% $\downarrow$}}& 3251.2\% $\uparrow$& 2779.5\% $\uparrow$& \textcolor{blue}{\textbf{44.1\% $\downarrow$}}& 0.6\% $\uparrow$& \textcolor{blue}{\textbf{0.2\% $\downarrow$}}& \textcolor{blue}{\textbf{83.9\% $\downarrow$}}& 26.4\% $\uparrow$& 16.7\% $\uparrow$& \textcolor{blue}{\textbf{78.8\% $\downarrow$}}& 4.4\% $\uparrow$& 5.3\% $\uparrow$& \textcolor{blue}{\textbf{85.2\% $\downarrow$}}& 3029.3\% $\uparrow$& 2621.3\% $\uparrow$& \textcolor{blue}{\textbf{44.3\% $\downarrow$}} \\
\midrule

Autoformer& \textbf{0.236}& \textbf{0.342}& \textbf{12.1}& \textbf{0.334}& \textbf{0.371}& 10.5& 0.583& 0.531& 10.5& \textbf{3.084}& \textbf{1.181}& 10.5& \textbf{0.639}& \textbf{0.397}& 14.9& \textbf{0.338}& \textbf{0.380}& 10.6 \\
+PALS& \textbf{nan}& \textbf{nan}& \textbf{nan}& 10.000& 10.000& \textbf{10.0}& \textbf{0.564}& \textbf{0.529}& \textbf{3.9}& 3.598& 1.318& \textbf{2.7}& 0.674& 0.420& \textbf{2.7}& 10.000& 10.000& \textbf{10.0} \\
Difference& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& 2896.1\% $\uparrow$& 2598.0\% $\uparrow$& \textcolor{blue}{\textbf{5.1\% $\downarrow$}}& \textcolor{blue}{\textbf{3.3\% $\downarrow$}}& \textcolor{blue}{\textbf{0.3\% $\downarrow$}}& \textcolor{blue}{\textbf{63.2\% $\downarrow$}}& 16.7\% $\uparrow$& 11.5\% $\uparrow$& \textcolor{blue}{\textbf{74.2\% $\downarrow$}}& 5.5\% $\uparrow$& 5.7\% $\uparrow$& \textcolor{blue}{\textbf{81.8\% $\downarrow$}}& 2854.9\% $\uparrow$& 2531.7\% $\uparrow$& \textcolor{blue}{\textbf{5.7\% $\downarrow$}} \\
\midrule

Informer& \textbf{0.356}& \textbf{0.433}& 12.5& 1.526& 0.881& 11.3& 1.593& 0.998& 11.3& \textbf{5.271}& \textbf{1.582}& 11.3& \textbf{0.811}& \textbf{0.456}& \textbf{14.4}& 0.620& 0.552& 11.4 \\
+PALS& 10.000& 10.000& \textbf{10.0}& \textbf{1.274}& \textbf{0.814}& \textbf{2.0}& \textbf{1.547}& \textbf{0.993}& \textbf{4.3}& 5.365& 1.589& \textbf{3.2}& \textbf{nan}& \textbf{nan}& \textbf{nan}& \textbf{0.388}& \textbf{0.426}& \textbf{0.0} \\
Difference& 2706.0\% $\uparrow$& 2208.6\% $\uparrow$& \textcolor{blue}{\textbf{19.7\% $\downarrow$}}& \textcolor{blue}{\textbf{16.5\% $\downarrow$}}& \textcolor{blue}{\textbf{7.7\% $\downarrow$}}& \textcolor{blue}{\textbf{81.9\% $\downarrow$}}& \textcolor{blue}{\textbf{2.9\% $\downarrow$}}& \textcolor{blue}{\textbf{0.5\% $\downarrow$}}& \textcolor{blue}{\textbf{61.8\% $\downarrow$}}& 1.8\% $\uparrow$& 0.4\% $\uparrow$& \textcolor{blue}{\textbf{71.9\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{37.4\% $\downarrow$}}& \textcolor{blue}{\textbf{22.9\% $\downarrow$}}& \textcolor{blue}{\textbf{99.8\% $\downarrow$}} \\
\midrule

Transformer& \textbf{0.281}& \textbf{0.375}& 11.7& \textbf{1.479}& \textbf{0.860}& 10.5& 1.609& 0.971& 10.5& \textbf{4.942}& \textbf{1.489}& 10.5& \textbf{0.667}& \textbf{0.361}& 13.6& \textbf{0.645}& \textbf{0.562}& \textbf{10.6} \\
+PALS& 10.000& 10.000& \textbf{10.0}& 10.000& 10.000& \textbf{10.0}& \textbf{1.337}& \textbf{0.899}& \textbf{3.5}& 5.111& 1.506& \textbf{3.1}& 10.000& 10.000& \textbf{10.0}& \textbf{nan}& \textbf{nan}& \textbf{nan} \\
Difference& 3456.2\% $\uparrow$& 2566.6\% $\uparrow$& \textcolor{blue}{\textbf{14.3\% $\downarrow$}}& 576.2\% $\uparrow$& 1063.3\% $\uparrow$& \textcolor{blue}{\textbf{5.1\% $\downarrow$}}& \textcolor{blue}{\textbf{16.9\% $\downarrow$}}& \textcolor{blue}{\textbf{7.4\% $\downarrow$}}& \textcolor{blue}{\textbf{66.6\% $\downarrow$}}& 3.4\% $\uparrow$& 1.1\% $\uparrow$& \textcolor{blue}{\textbf{70.9\% $\downarrow$}}& 1400.2\% $\uparrow$& 2668.2\% $\uparrow$& \textcolor{blue}{\textbf{26.5\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}} \\
\midrule

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{19}{c}{Sparse Model Hidden Size = 512, Init Density = 1}\\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
NSTransformer& \textbf{0.194}& \textbf{0.296}& 11.9& 0.505& 0.438& 10.7& 0.541& 0.487& 10.6& \textbf{2.138}& \textbf{0.919}& 10.5& \textbf{0.632}& \textbf{0.344}& 14.1& 0.292& 0.313& 10.6 \\
+PALS& 0.214& 0.317& \textbf{2.2}& \textbf{0.384}& \textbf{0.387}& \textbf{2.7}& \textbf{0.539}& \textbf{0.483}& \textbf{6.0}& 2.324& 0.969& \textbf{6.9}& 0.666& 0.375& \textbf{4.3}& \textbf{0.260}& \textbf{0.288}& \textbf{1.1} \\
Difference& 10.4\% $\uparrow$& 7.1\% $\uparrow$& \textcolor{blue}{\textbf{81.5\% $\downarrow$}}& \textcolor{blue}{\textbf{23.9\% $\downarrow$}}& \textcolor{blue}{\textbf{11.6\% $\downarrow$}}& \textcolor{blue}{\textbf{74.8\% $\downarrow$}}& \textcolor{blue}{\textbf{0.5\% $\downarrow$}}& \textcolor{blue}{\textbf{0.9\% $\downarrow$}}& \textcolor{blue}{\textbf{42.8\% $\downarrow$}}& 8.7\% $\uparrow$& 5.5\% $\uparrow$& \textcolor{blue}{\textbf{34.1\% $\downarrow$}}& 5.4\% $\uparrow$& 9.2\% $\uparrow$& \textcolor{blue}{\textbf{69.3\% $\downarrow$}}& \textcolor{blue}{\textbf{10.9\% $\downarrow$}}& \textcolor{blue}{\textbf{8.1\% $\downarrow$}}& \textcolor{blue}{\textbf{90.1\% $\downarrow$}} \\
\midrule

FEDformer& \textbf{0.207}& \textbf{0.321}& 19.5& 0.298& 0.347& 17.9& \textbf{0.501}& \textbf{0.493}& 17.9& \textbf{2.840}& \textbf{1.137}& 14.3& \textbf{0.609}& \textbf{0.377}& 22.3& 0.320& 0.367& 17.9 \\
+PALS& 0.229& 0.338& \textbf{4.2}& \textbf{0.297}& \textbf{0.340}& \textbf{1.0}& 0.512& 0.499& \textbf{10.6}& 3.030& 1.189& \textbf{8.1}& 0.616& 0.381& \textbf{6.0}& \textbf{0.309}& \textbf{0.354}& \textbf{1.0} \\
Difference& 10.3\% $\uparrow$& 5.6\% $\uparrow$& \textcolor{blue}{\textbf{78.7\% $\downarrow$}}& \textcolor{blue}{\textbf{0.5\% $\downarrow$}}& \textcolor{blue}{\textbf{2.1\% $\downarrow$}}& \textcolor{blue}{\textbf{94.6\% $\downarrow$}}& 2.2\% $\uparrow$& 1.2\% $\uparrow$& \textcolor{blue}{\textbf{40.9\% $\downarrow$}}& 6.7\% $\uparrow$& 4.5\% $\uparrow$& \textcolor{blue}{\textbf{43.0\% $\downarrow$}}& 1.0\% $\uparrow$& 1.2\% $\uparrow$& \textcolor{blue}{\textbf{73.0\% $\downarrow$}}& \textcolor{blue}{\textbf{3.4\% $\downarrow$}}& \textcolor{blue}{\textbf{3.7\% $\downarrow$}}& \textcolor{blue}{\textbf{94.5\% $\downarrow$}} \\
\midrule

Autoformer& \textbf{0.236}& \textbf{0.342}& 12.1& 0.334& 0.371& 10.5& \textbf{0.583}& \textbf{0.531}& 10.5& \textbf{3.084}& \textbf{1.181}& 10.5& \textbf{0.639}& \textbf{0.397}& 14.9& 0.338& 0.380& 10.6 \\
+PALS& 0.250& 0.353& \textbf{3.6}& \textbf{0.305}& \textbf{0.348}& \textbf{0.7}& 0.608& 0.547& \textbf{7.9}& 3.239& 1.230& \textbf{6.3}& 0.651& 0.405& \textbf{4.8}& \textbf{0.328}& \textbf{0.365}& \textbf{1.1} \\
Difference& 6.1\% $\uparrow$& 3.2\% $\uparrow$& \textcolor{blue}{\textbf{70.2\% $\downarrow$}}& \textcolor{blue}{\textbf{8.6\% $\downarrow$}}& \textcolor{blue}{\textbf{6.1\% $\downarrow$}}& \textcolor{blue}{\textbf{93.4\% $\downarrow$}}& 4.3\% $\uparrow$& 3.2\% $\uparrow$& \textcolor{blue}{\textbf{25.3\% $\downarrow$}}& 5.0\% $\uparrow$& 4.1\% $\uparrow$& \textcolor{blue}{\textbf{40.6\% $\downarrow$}}& 1.9\% $\uparrow$& 2.1\% $\uparrow$& \textcolor{blue}{\textbf{67.7\% $\downarrow$}}& \textcolor{blue}{\textbf{3.1\% $\downarrow$}}& \textcolor{blue}{\textbf{4.0\% $\downarrow$}}& \textcolor{blue}{\textbf{89.6\% $\downarrow$}} \\
\midrule

Informer& \textbf{0.356}& \textbf{0.433}& 12.5& 1.526& 0.881& 11.3& 1.593& 0.998& 11.3& 5.271& 1.582& 11.3& \textbf{0.811}& \textbf{0.456}& 14.4& 0.620& 0.552& 11.4 \\
+PALS& 0.436& 0.489& \textbf{1.4}& \textbf{1.464}& \textbf{0.853}& \textbf{6.8}& \textbf{1.566}& \textbf{0.992}& \textbf{9.5}& \textbf{5.209}& \textbf{1.560}& \textbf{7.3}& 0.934& 0.525& \textbf{2.3}& \textbf{0.326}& \textbf{0.374}& \textbf{0.7} \\
Difference& 22.3\% $\uparrow$& 13.0\% $\uparrow$& \textcolor{blue}{\textbf{88.8\% $\downarrow$}}& \textcolor{blue}{\textbf{4.1\% $\downarrow$}}& \textcolor{blue}{\textbf{3.1\% $\downarrow$}}& \textcolor{blue}{\textbf{40.2\% $\downarrow$}}& \textcolor{blue}{\textbf{1.7\% $\downarrow$}}& \textcolor{blue}{\textbf{0.6\% $\downarrow$}}& \textcolor{blue}{\textbf{16.4\% $\downarrow$}}& \textcolor{blue}{\textbf{1.2\% $\downarrow$}}& \textcolor{blue}{\textbf{1.4\% $\downarrow$}}& \textcolor{blue}{\textbf{35.6\% $\downarrow$}}& 15.2\% $\uparrow$& 15.2\% $\uparrow$& \textcolor{blue}{\textbf{83.8\% $\downarrow$}}& \textcolor{blue}{\textbf{47.3\% $\downarrow$}}& \textcolor{blue}{\textbf{32.2\% $\downarrow$}}& \textcolor{blue}{\textbf{93.5\% $\downarrow$}} \\
\midrule

Transformer& \textbf{0.281}& \textbf{0.375}& 11.7& 1.479& 0.860& 10.5& 1.609& 0.971& 10.5& 4.942& 1.489& 10.5& \textbf{0.667}& \textbf{0.361}& 13.6& 0.645& 0.562& 10.6 \\
+PALS& 0.311& 0.397& \textbf{3.1}& \textbf{1.190}& \textbf{0.750}& \textbf{8.1}& \textbf{1.333}& \textbf{0.890}& \textbf{7.8}& \textbf{4.916}& \textbf{1.477}& \textbf{7.9}& 0.688& 0.381& \textbf{3.8}& \textbf{0.263}& \textbf{0.326}& \textbf{0.3} \\
Difference& 10.8\% $\uparrow$& 5.9\% $\uparrow$& \textcolor{blue}{\textbf{73.2\% $\downarrow$}}& \textcolor{blue}{\textbf{19.5\% $\downarrow$}}& \textcolor{blue}{\textbf{12.7\% $\downarrow$}}& \textcolor{blue}{\textbf{23.3\% $\downarrow$}}& \textcolor{blue}{\textbf{17.2\% $\downarrow$}}& \textcolor{blue}{\textbf{8.3\% $\downarrow$}}& \textcolor{blue}{\textbf{26.4\% $\downarrow$}}& \textcolor{blue}{\textbf{0.5\% $\downarrow$}}& \textcolor{blue}{\textbf{0.8\% $\downarrow$}}& \textcolor{blue}{\textbf{25.0\% $\downarrow$}}& 3.3\% $\uparrow$& 5.4\% $\uparrow$& \textcolor{blue}{\textbf{71.7\% $\downarrow$}}& \textcolor{blue}{\textbf{59.2\% $\downarrow$}}& \textcolor{blue}{\textbf{42.0\% $\downarrow$}}& \textcolor{blue}{\textbf{97.0\% $\downarrow$}} \\







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
\multicolumn{19}{c}{Sparse Model Hidden Size = 768, Init Density = 0.5}\\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
NSTransformer& \textbf{0.194}& \textbf{0.296}& 11.9& 0.505& 0.438& 10.7& \textbf{0.541}& \textbf{0.487}& 10.6& \textbf{2.138}& \textbf{0.919}& 10.5& \textbf{0.632}& \textbf{0.344}& 14.1& 0.292& 0.313& 10.6 \\
+PALS& 0.220& 0.322& \textbf{2.8}& \textbf{0.417}& \textbf{0.403}& \textbf{4.5}& 0.579& 0.494& \textbf{9.7}& 2.578& 1.027& \textbf{6.2}& 0.665& 0.376& \textbf{4.0}& \textbf{0.253}& \textbf{0.284}& \textbf{0.2} \\
Difference& 13.4\% $\uparrow$& 8.8\% $\uparrow$& \textcolor{blue}{\textbf{76.7\% $\downarrow$}}& \textcolor{blue}{\textbf{17.5\% $\downarrow$}}& \textcolor{blue}{\textbf{7.9\% $\downarrow$}}& \textcolor{blue}{\textbf{57.8\% $\downarrow$}}& 7.1\% $\uparrow$& 1.5\% $\uparrow$& \textcolor{blue}{\textbf{8.2\% $\downarrow$}}& 20.6\% $\uparrow$& 11.8\% $\uparrow$& \textcolor{blue}{\textbf{41.0\% $\downarrow$}}& 5.1\% $\uparrow$& 9.5\% $\uparrow$& \textcolor{blue}{\textbf{71.4\% $\downarrow$}}& \textcolor{blue}{\textbf{13.2\% $\downarrow$}}& \textcolor{blue}{\textbf{9.3\% $\downarrow$}}& \textcolor{blue}{\textbf{98.3\% $\downarrow$}} \\
\midrule

FEDformer& \textbf{0.207}& \textbf{0.321}& 19.5& \textbf{0.298}& \textbf{0.347}& \textbf{17.9}& \textbf{0.501}& \textbf{0.493}& 17.9& \textbf{2.840}& \textbf{1.137}& 14.3& \textbf{0.609}& \textbf{0.377}& 22.3& 0.320& 0.367& 17.9 \\
+PALS& 0.279& 0.374& \textbf{3.9}& \textbf{nan}& \textbf{nan}& \textbf{nan}& 0.528& 0.506& \textbf{10.6}& 3.248& 1.247& \textbf{6.9}& 0.644& 0.404& \textbf{4.7}& \textbf{0.313}& \textbf{0.357}& \textbf{0.9} \\
Difference& 34.6\% $\uparrow$& 16.7\% $\uparrow$& \textcolor{blue}{\textbf{80.2\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& 5.4\% $\uparrow$& 2.6\% $\uparrow$& \textcolor{blue}{\textbf{40.7\% $\downarrow$}}& 14.4\% $\uparrow$& 9.7\% $\uparrow$& \textcolor{blue}{\textbf{51.9\% $\downarrow$}}& 5.7\% $\uparrow$& 7.3\% $\uparrow$& \textcolor{blue}{\textbf{78.7\% $\downarrow$}}& \textcolor{blue}{\textbf{2.0\% $\downarrow$}}& \textcolor{blue}{\textbf{2.8\% $\downarrow$}}& \textcolor{blue}{\textbf{95.2\% $\downarrow$}} \\
\midrule

Autoformer& \textbf{0.236}& \textbf{0.342}& 12.1& \textbf{0.334}& \textbf{0.371}& 10.5& 0.583& 0.531& 10.5& \textbf{3.084}& \textbf{1.181}& 10.5& \textbf{0.639}& \textbf{0.397}& 14.9& \textbf{0.338}& \textbf{0.380}& \textbf{10.6} \\
+PALS& 0.248& 0.347& \textbf{3.3}& 10.000& 10.000& \textbf{10.0}& \textbf{0.521}& \textbf{0.506}& \textbf{7.5}& 3.451& 1.284& \textbf{4.9}& 0.677& 0.422& \textbf{3.7}& \textbf{nan}& \textbf{nan}& \textbf{nan} \\
Difference& 5.1\% $\uparrow$& 1.2\% $\uparrow$& \textcolor{blue}{\textbf{72.9\% $\downarrow$}}& 2896.1\% $\uparrow$& 2598.0\% $\uparrow$& \textcolor{blue}{\textbf{5.1\% $\downarrow$}}& \textcolor{blue}{\textbf{10.7\% $\downarrow$}}& \textcolor{blue}{\textbf{4.6\% $\downarrow$}}& \textcolor{blue}{\textbf{28.5\% $\downarrow$}}& 11.9\% $\uparrow$& 8.7\% $\uparrow$& \textcolor{blue}{\textbf{53.7\% $\downarrow$}}& 6.0\% $\uparrow$& 6.3\% $\uparrow$& \textcolor{blue}{\textbf{75.1\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}} \\
\midrule

Informer& \textbf{0.356}& \textbf{0.433}& 12.5& 1.526& 0.881& 11.3& 1.593& 0.998& 11.3& 5.271& 1.582& 11.3& \textbf{0.811}& \textbf{0.456}& 14.4& 0.620& 0.552& 11.4 \\
+PALS& 0.470& 0.514& \textbf{1.6}& \textbf{1.379}& \textbf{0.824}& \textbf{10.6}& \textbf{1.428}& \textbf{0.947}& \textbf{9.4}& \textbf{5.158}& \textbf{1.549}& \textbf{8.4}& 0.919& 0.516& \textbf{1.3}& \textbf{0.534}& \textbf{0.475}& \textbf{5.4} \\
Difference& 31.9\% $\uparrow$& 18.6\% $\uparrow$& \textcolor{blue}{\textbf{86.9\% $\downarrow$}}& \textcolor{blue}{\textbf{9.6\% $\downarrow$}}& \textcolor{blue}{\textbf{6.4\% $\downarrow$}}& \textcolor{blue}{\textbf{6.8\% $\downarrow$}}& \textcolor{blue}{\textbf{10.4\% $\downarrow$}}& \textcolor{blue}{\textbf{5.1\% $\downarrow$}}& \textcolor{blue}{\textbf{17.2\% $\downarrow$}}& \textcolor{blue}{\textbf{2.2\% $\downarrow$}}& \textcolor{blue}{\textbf{2.1\% $\downarrow$}}& \textcolor{blue}{\textbf{26.3\% $\downarrow$}}& 13.3\% $\uparrow$& 13.2\% $\uparrow$& \textcolor{blue}{\textbf{90.8\% $\downarrow$}}& \textcolor{blue}{\textbf{13.9\% $\downarrow$}}& \textcolor{blue}{\textbf{14.0\% $\downarrow$}}& \textcolor{blue}{\textbf{52.8\% $\downarrow$}} \\
\midrule

Transformer& \textbf{0.281}& \textbf{0.375}& \textbf{11.7}& \textbf{1.479}& \textbf{0.860}& \textbf{10.5}& 1.609& 0.971& 10.5& 4.942& 1.489& 10.5& \textbf{0.667}& \textbf{0.361}& 13.6& 0.645& 0.562& 10.6 \\
+PALS& \textbf{nan}& \textbf{nan}& \textbf{nan}& \textbf{nan}& \textbf{nan}& \textbf{nan}& \textbf{1.333}& \textbf{0.907}& \textbf{6.6}& \textbf{4.707}& \textbf{1.434}& \textbf{4.3}& 0.703& 0.392& \textbf{2.9}& \textbf{0.269}& \textbf{0.334}& \textbf{0.1} \\
Difference& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{17.2\% $\downarrow$}}& \textcolor{blue}{\textbf{6.5\% $\downarrow$}}& \textcolor{blue}{\textbf{37.1\% $\downarrow$}}& \textcolor{blue}{\textbf{4.8\% $\downarrow$}}& \textcolor{blue}{\textbf{3.7\% $\downarrow$}}& \textcolor{blue}{\textbf{59.5\% $\downarrow$}}& 5.5\% $\uparrow$& 8.6\% $\uparrow$& \textcolor{blue}{\textbf{78.7\% $\downarrow$}}& \textcolor{blue}{\textbf{58.3\% $\downarrow$}}& \textcolor{blue}{\textbf{40.5\% $\downarrow$}}& \textcolor{blue}{\textbf{99.4\% $\downarrow$}} \\



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
\multicolumn{19}{c}{Sparse Model Hidden Size = 768, Init Density = 1}\\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

NSTransformer& \textbf{0.194}& \textbf{0.296}& 11.9& 0.505& 0.438& \textbf{10.7}& \textbf{0.541}& \textbf{0.487}& \textbf{10.6}& \textbf{2.138}& \textbf{0.919}& \textbf{10.5}& \textbf{0.632}& \textbf{0.344}& 14.1& \textbf{0.292}& \textbf{0.313}& \textbf{10.6} \\
+PALS& 0.204& 0.307& \textbf{5.8}& \textbf{0.417}& \textbf{0.398}& 17.1& 0.584& 0.494& 18.9& 2.212& 0.932& 12.2& 0.645& 0.360& \textbf{6.9}& \textbf{nan}& \textbf{nan}& \textbf{nan} \\
Difference& 5.3\% $\uparrow$& 3.7\% $\uparrow$& \textcolor{blue}{\textbf{51.1\% $\downarrow$}}& \textcolor{blue}{\textbf{17.4\% $\downarrow$}}& \textcolor{blue}{\textbf{9.0\% $\downarrow$}}& 59.7\% $\uparrow$& 7.9\% $\uparrow$& 1.4\% $\uparrow$& 79.3\% $\uparrow$& 3.5\% $\uparrow$& 1.4\% $\uparrow$& 15.6\% $\uparrow$& 2.0\% $\uparrow$& 4.7\% $\uparrow$& \textcolor{blue}{\textbf{51.2\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}} \\
\midrule

FEDformer& \textbf{0.207}& \textbf{0.321}& 19.5& \textbf{0.298}& \textbf{0.347}& \textbf{17.9}& \textbf{0.501}& \textbf{0.493}& \textbf{17.9}& 2.840& 1.137& \textbf{14.3}& 0.609& 0.377& 22.3& 0.320& 0.367& 17.9 \\
+PALS& 0.220& 0.331& \textbf{8.9}& \textbf{nan}& \textbf{nan}& \textbf{nan}& 0.526& 0.505& 26.8& \textbf{2.767}& \textbf{1.120}& 15.4& \textbf{0.609}& \textbf{0.376}& \textbf{10.8}& \textbf{0.304}& \textbf{0.350}& \textbf{0.6} \\
Difference& 6.0\% $\uparrow$& 3.2\% $\uparrow$& \textcolor{blue}{\textbf{54.5\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& 5.1\% $\uparrow$& 2.4\% $\uparrow$& 49.8\% $\uparrow$& \textcolor{blue}{\textbf{2.6\% $\downarrow$}}& \textcolor{blue}{\textbf{1.5\% $\downarrow$}}& 7.7\% $\uparrow$& \textcolor{blue}{\textbf{0.1\% $\downarrow$}}& \textcolor{blue}{\textbf{0.1\% $\downarrow$}}& \textcolor{blue}{\textbf{51.5\% $\downarrow$}}& \textcolor{blue}{\textbf{5.0\% $\downarrow$}}& \textcolor{blue}{\textbf{4.7\% $\downarrow$}}& \textcolor{blue}{\textbf{96.8\% $\downarrow$}} \\
\midrule

Autoformer& \textbf{0.236}& \textbf{0.342}& 12.1& \textbf{0.334}& \textbf{0.371}& 10.5& 0.583& 0.531& \textbf{10.5}& 3.084& 1.181& \textbf{10.5}& 0.639& 0.397& 14.9& \textbf{0.338}& \textbf{0.380}& 10.6 \\
+PALS& 0.238& 0.344& \textbf{3.2}& 10.000& 10.000& \textbf{10.0}& \textbf{0.562}& \textbf{0.528}& 12.0& \textbf{2.970}& \textbf{1.163}& 13.6& \textbf{0.633}& \textbf{0.393}& \textbf{7.3}& 10.000& 10.000& \textbf{10.0} \\
Difference& 0.9\% $\uparrow$& 0.6\% $\uparrow$& \textcolor{blue}{\textbf{73.3\% $\downarrow$}}& 2896.1\% $\uparrow$& 2598.0\% $\uparrow$& \textcolor{blue}{\textbf{5.1\% $\downarrow$}}& \textcolor{blue}{\textbf{3.6\% $\downarrow$}}& \textcolor{blue}{\textbf{0.6\% $\downarrow$}}& 13.9\% $\uparrow$& \textcolor{blue}{\textbf{3.7\% $\downarrow$}}& \textcolor{blue}{\textbf{1.6\% $\downarrow$}}& 29.0\% $\uparrow$& \textcolor{blue}{\textbf{1.0\% $\downarrow$}}& \textcolor{blue}{\textbf{1.0\% $\downarrow$}}& \textcolor{blue}{\textbf{50.8\% $\downarrow$}}& 2854.9\% $\uparrow$& 2531.7\% $\uparrow$& \textcolor{blue}{\textbf{5.7\% $\downarrow$}} \\
\midrule

Informer& \textbf{0.356}& \textbf{0.433}& 12.5& 1.526& 0.881& \textbf{11.3}& 1.593& 0.998& \textbf{11.3}& \textbf{5.271}& \textbf{1.582}& \textbf{11.3}& 0.811& 0.456& 14.4& 0.620& 0.552& 11.4 \\
+PALS& 0.371& 0.446& \textbf{1.2}& \textbf{1.465}& \textbf{0.858}& 20.0& \textbf{1.556}& \textbf{0.984}& 18.8& 5.277& 1.583& 17.5& \textbf{0.793}& \textbf{0.450}& \textbf{3.2}& \textbf{0.311}& \textbf{0.370}& \textbf{0.4} \\
Difference& 4.1\% $\uparrow$& 2.9\% $\uparrow$& \textcolor{blue}{\textbf{90.1\% $\downarrow$}}& \textcolor{blue}{\textbf{4.0\% $\downarrow$}}& \textcolor{blue}{\textbf{2.6\% $\downarrow$}}& 76.7\% $\uparrow$& \textcolor{blue}{\textbf{2.3\% $\downarrow$}}& \textcolor{blue}{\textbf{1.4\% $\downarrow$}}& 65.7\% $\uparrow$& 0.1\% $\uparrow$& 0.0\% $\uparrow$& 54.9\% $\uparrow$& \textcolor{blue}{\textbf{2.3\% $\downarrow$}}& \textcolor{blue}{\textbf{1.4\% $\downarrow$}}& \textcolor{blue}{\textbf{77.9\% $\downarrow$}}& \textcolor{blue}{\textbf{49.7\% $\downarrow$}}& \textcolor{blue}{\textbf{33.0\% $\downarrow$}}& \textcolor{blue}{\textbf{96.2\% $\downarrow$}} \\
\midrule

Transformer& \textbf{0.281}& \textbf{0.375}& \textbf{11.7}& \textbf{1.479}& \textbf{0.860}& 10.5& 1.609& 0.971& \textbf{10.5}& 4.942& 1.489& \textbf{10.5}& \textbf{0.667}& \textbf{0.361}& \textbf{13.6}& \textbf{0.645}& \textbf{0.562}& \textbf{10.6} \\
+PALS& \textbf{nan}& \textbf{nan}& \textbf{nan}& 10.000& 10.000& \textbf{10.0}& \textbf{1.452}& \textbf{0.936}& 17.8& \textbf{4.799}& \textbf{1.459}& 13.1& \textbf{nan}& \textbf{nan}& \textbf{nan}& \textbf{nan}& \textbf{nan}& \textbf{nan} \\
Difference& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& 576.2\% $\uparrow$& 1063.3\% $\uparrow$& \textcolor{blue}{\textbf{5.1\% $\downarrow$}}& \textcolor{blue}{\textbf{9.8\% $\downarrow$}}& \textcolor{blue}{\textbf{3.6\% $\downarrow$}}& 69.1\% $\uparrow$& \textcolor{blue}{\textbf{2.9\% $\downarrow$}}& \textcolor{blue}{\textbf{2.1\% $\downarrow$}}& 24.2\% $\uparrow$& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}}& \textcolor{blue}{\textbf{nan\% $\downarrow$}} \\
\bottomrule
\end{tabular}}
\end{center}
\end{scriptsize}

\end{table*}


==> assets/tables/table_ks.tex <==

\begin{table*}[!b]




\caption{Two-sample Kolmogorov-Smirnov test results. We compare the underlying distributions of the prediction and the ground truth for each dataset and model. }\label{tab:results_ks}
\vspace{-3mm}
\centering
\resizebox{0.6\textwidth}{!}{% <------ Don't forget this %
\begin{tabular}{c|c|cc|cc|cc|cc|cc}
\toprule
& \bt \multirow{3}{*}{$H$} &\multicolumn{2}{c}{NSTransformer} &\multicolumn{2}{c}{FEDformer} &\multicolumn{2}{c}{Autoformer}&\multicolumn{2}{c}{Informer} &\multicolumn{2}{c}{Transformer}\\

&&Dense &PALS &Dense &PALS  &Dense &PALS &Dense &PALS &Dense &PALS\\ 
\midrule


\multirow{4}{*}{\rotatebox[origin=c]{90}{Electricity}}& 96& \pmb{70.8792}& 75.1635& 74.3342& 77.7916& 77.5635& 79.5410& 97.5615& 101.0985& 87.5790& 91.7447 \\
& 192& \pmb{105.2581}& 110.3782& 108.7820& 113.9496& 116.1705& 117.6647& 142.1929& 149.4319& 125.9163& 136.1502 \\
& 336& \pmb{142.7428}& 151.0012& 149.3587& 155.6534& 155.7136& 168.9656& 191.6481& 208.6804& 172.8792& 184.8464 \\
& 720& 0.0000& \textcolor{blue}{\pmb{235.0201}}& 0.0000& 255.6771& 0.0000& 286.5808& 0.0000& 342.9665& 0.0000& 278.2182 \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETTm2}}& 96& 10.1693& 11.6192& \pmb{9.3307}& 9.4678& 10.9023& \textcolor{blue}{9.9614}& 17.9967& \textcolor{blue}{15.5591}& 14.4305& \textcolor{blue}{13.0194} \\
& 192& 18.6567& \textcolor{blue}{16.5569}& \pmb{15.0567}& 15.2195& 15.8328& \textcolor{blue}{15.7870}& 28.7961& \textcolor{blue}{28.2980}& 33.2964& \textcolor{blue}{25.7116} \\
& 336& 29.1511& \textcolor{blue}{23.6227}& \pmb{21.8081}& 21.9224& 23.2092& \textcolor{blue}{22.5953}& 54.1095& \textcolor{blue}{47.6077}& 53.0797& \textcolor{blue}{43.9828} \\
& 720& 0.0000& \textcolor{blue}{\pmb{23.6227}}& 0.0000& \textcolor{blue}{\pmb{23.6227}}& 0.0000& \textcolor{blue}{\pmb{23.6227}}& 0.0000& \textcolor{blue}{\pmb{23.6227}}& 0.0000& \textcolor{blue}{\pmb{23.6227}} \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Exchange}}& 96& \pmb{8.8643}& 9.4544& 9.9489& 10.2978& 9.7514& 10.0153& 26.3124& 26.4792& 0.0& 0.0 \\
& 192& 18.6869& \textcolor{blue}{\pmb{18.5704}}& 18.8939& 19.2082& 19.5286& 19.9300& 39.1016& 39.3367& 0.0& 0.0 \\
& 336& 30.3562& 32.0045& 32.1385& \textcolor{blue}{32.0881}& 51.3789& \textcolor{blue}{34.4071}& 0.0000& \textcolor{blue}{\pmb{18.5704}}& 0.0& 0.0 \\
& 720& 79.8050& 80.4755& 78.9801& \textcolor{blue}{78.3751}& \pmb{78.0222}& 79.8495& 109.4899& 113.3798& 0.0& 0.0 \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Illness}}& 24& \pmb{16.7656}& 17.8975& 20.4539& 21.8311& 21.0857& 22.6592& 25.1654& 25.2867& 24.5829& 24.8186 \\
& 36& \pmb{19.2479}& 20.6023& 21.5868& 22.3878& 22.4026& 25.2115& 30.1537& \textcolor{blue}{30.0708}& 30.9906& 31.0165 \\
& 48& \pmb{23.1604}& 25.2256& 24.8849& 26.4836& 28.0617& 29.1677& 35.7298& 35.7886& 36.7398& \textcolor{blue}{36.4722} \\
& 60& \pmb{28.2417}& 30.1003& 28.5556& 30.0882& 30.6525& 32.4039& 40.5608& 40.8863& 43.5080& \textcolor{blue}{43.1519} \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Traffic}}& 96& 219.4518& 223.5573& \pmb{215.4409}& 216.5813& 225.1615& \textcolor{blue}{219.3979}& 233.8757& 239.7220& 223.1035& 228.1622 \\
& 192& 315.5887& 320.4817& \pmb{308.3012}& 311.1115& 313.1786& 315.3727& 334.2745& 342.5088& 320.7737& 326.5867 \\
& 336& 425.1846& \textcolor{blue}{422.9549}& 411.3128& 415.5384& \pmb{411.2185}& 421.7124& 454.5023& 494.5789& 423.4712& 429.3374 \\
& 720& \pmb{425.1846}& 628.4570& \pmb{425.1846}& 616.1093& \pmb{425.1846}& 619.9954& \pmb{425.1846}& 806.6493& \pmb{425.1846}& 640.5836 \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Weather}}& 96& 16.7286& \textcolor{blue}{\pmb{16.5881}}& 21.3003& \textcolor{blue}{19.5352}& 20.6789& \textcolor{blue}{20.3924}& 25.6817& \textcolor{blue}{22.6239}& 23.8817& \textcolor{blue}{17.5991} \\
& 192& 28.3624& \textcolor{blue}{\pmb{27.3050}}& 31.6057& 31.9208& 31.8981& \textcolor{blue}{31.8902}& 37.9879& \textcolor{blue}{35.4127}& 45.2360& \textcolor{blue}{31.4975} \\
& 336& 44.0638& \textcolor{blue}{\pmb{41.8018}}& 44.8369& 44.9520& 45.4612& 45.5895& 60.4263& \textcolor{blue}{56.2232}& 63.4263& \textcolor{blue}{47.8726} \\
& 720& 0.0000& \textcolor{blue}{\pmb{41.8018}}& 0.0000& \textcolor{blue}{\pmb{41.8018}}& 0.0000& \textcolor{blue}{\pmb{41.8018}}& 0.0000& \textcolor{blue}{\pmb{41.8018}}& 0.0000& \textcolor{blue}{\pmb{41.8018}} \\
\midrule
\bottomrule
\end{tabular}}


\end{table*}




